A Bilevel Optimization Scheme for Persistent Monitoring

In this paper we study an infinite-horizon persistent monitoring problem in a two-dimensional mission space containing a finite number of statically placed targets, at each of which we assume a constant rate of uncertainty accumulation. Equipped with a sensor of finite range, the agent is capable of reducing the uncertainty of nearby targets. We derive a steady-state minimum time periodic trajectory over which each of the target uncertainties is driven down to zero during each visit. A hierarchical decomposition leads to purely local optimal control problems, coupled via boundary conditions. We optimize both the local trajectory segments as well as the boundary conditions in an on-line bilevel optimization scheme.

==> OL_latex_setup/cite.tex <==

\usepackage{cite}


==> OL_latex_setup/generic_beamer_setup.tex <==
\input{\SETUPDIR/generic_setup.tex}

\usepackage[style=numeric, 
            backend=biber,
            giveninits=true]{biblatex}

\addbibresource{\BIBTEXDIR/biblio.bib}


\DeclareFieldFormat{beamercolorauthor}{%
  \usebeamercolor[fg]{bibliography entry author}%
  #1}
\DeclareFieldFormat{beamercolortitle}{%
  \usebeamercolor[fg]{bibliography entry title}%
  #1}
\DeclareFieldFormat{beamercolornote}{%
  \usebeamercolor[fg]{bibliography entry note}%
  #1}

\DeclareCiteCommand{\fullcite}
  {\usebibmacro{prenote}}
  {\printtext[beamercolorauthor]{%
     \printnames[given-family]{labelname}%
     \setunit{\addcomma\space}}%
   \printtext[beamercolornote]{%
     \printfield{journaltitle}%
     \printfield{booktitle}%
     \setunit{\addspace}%
     \printtext[parens]{%
       \printdate}}}
  {\multicitedelim}
  {\usebibmacro{postnote}}

  \newcommand{\citeColored}[2]{{\hypersetup{citecolor=#1}\fullcite{‌​#2}}}


==> OL_latex_setup/iguana_setup.tex <==
% Packages
\usepackage{cite}
\usepackage{amssymb,amsfonts}


==> OL_latex_setup/tikz_setup.tex <==

%% Tikz
\usepackage{tikz}
\usetikzlibrary{positioning, arrows, calc, arrows.meta}

\tikzset{
	%Define standard arrow tip
	>=stealth',
	%Define style for different line styles
	help lines/.style={dashed, thick},
	axis/.style={<->},
	important line/.style={thick},
	connection/.style={thick, dotted},
}

%% PGF plots
\usepackage{pgfplots, pgfplotstable}
\pgfplotsset{compat=1.16}
\newlength\fheight
\newlength\fwidth
\setlength\fheight{4cm}
\setlength\fwidth{6cm}


==> OL_latex_setup/xcolor.tex <==
\usepackage[dvipsnames]{xcolor}


==> sections/adaptations.tex <==
\section{Extensions and Adaptations}\label{sec:high:level:solutions}

\subsection{Extending to Mobile Targets}
\begin{itemize}
    \item The low level optimization problem can be extended to a mobile target easily by simply augmenting the state space.
    \item If the target dynamics are unknown then we should use an MPC controller for this stage
    \item Note that the constant control from the switch between visited targets in the static case simply resulted from the minimum time switching control. In the case of mobile targets we can simply solve another time optimal traveling problem including the target dynamics (or MPC if dynamics are uncertain).
    \item Can we prove convergence to some steady-state policy under certain periodicity assumptions of the targets' dynamics?
\end{itemize}

\subsection{Adapting to higher-order dynamics}
\begin{itemize}
    \item The switching control during a switch is already constant, i.e., smooth.
    \item The low level controller can be adapted easily to account for higher order dynamics
    \item Glueing the pieces together can lead to second-order infeasibility. 
    \item We simply need more initial and terminal constraints for the lower level controller that enforces transition smoothness.
\end{itemize}

\subsection{Optimizing the visiting sequence}
\begin{itemize}
    \item Estimate the average drain rate for each target given an uncertainty value
    \item Then abstract the network to a graph and use a high level controller such as~\cite{welikala2021event} to obtain visiting sequences.
\end{itemize}

\subsection{Adapting to Multi-Agent Scenarios}
\begin{itemize}
    \item The method should easily extend to (centralized) multi-agent scenarios
    \item Each agent has its own controller
\end{itemize}


==> sections/deprecated_figures.tex <==
\section{Deprecated Figures}

\begin{figure}
    \centering
    \includegraphics[width=0.95\linewidth]{figures/illustrations/hierarchies_zoomed/hierarchies_zoomed.pdf}
    \caption{Illustration of the high level problem of determining a visiting sequence (left) and the low level draining problem (right) with entrance point (blue) and departure point (green). }
    \label{fig:deprecated:depicted:hierarchies}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/illustrations/hierarchies/hierarchies.pdf}
    \caption{}
    \label{fig:deprecated:hierarchies}
\end{figure}
